How Well Do My Results Generalize Now? The External Validity of Online Privacy and Security Surveys

Privacy and security researchers often rely on data collected through online crowdsourcing platforms such as Amazon Mechanical Turk (MTurk) and Prolific. Prior work -- which used data collected in the United States between 2013 and 2017 -- found that MTurk responses regarding security and privacy were generally representative for people under 50 or with some college education. However, the landscape of online crowdsourcing has changed significantly over the last five years, with the rise of Prolific as a major platform and the increasing presence of bots. This work attempts to replicate the prior results about the external validity of online privacy and security surveys. We conduct an online survey on MTurk (n=800), a gender-balanced survey on Prolific (n=800), and a representative survey on Prolific (n=800) and compare the responses to a probabilistic survey conducted by the Pew Research Center (n=4272). We find that MTurk response quality has degraded over the last five years, and our results do not replicate the earlier finding about the generalizability of MTurk responses. By contrast, we find that data collected through Prolific is generally representative for questions about user perceptions and experiences, but not for questions about security and privacy knowledge. We also evaluate the impact of Prolific settings, attention check questions, and statistical methods on the external validity of online surveys, and we develop recommendations about best practices for conducting online privacy and security surveys.

==> sections/xxx_scrap.tex <==
    \subsubsection{Unfiltered} 
    Table~\ref{tab:mturk} shows that for all but one question, responses from MTurkers were distributed differently than responses from the representative Pew survey. The distributions of answers from MTurkers are not only \textit{statistically} different than those that Pew found nationally, but their \textit{magnitude} of difference is very large. Table~\ref{mturk} also shows that the magnitude of these differences are at times enormous: the difference in the percentage of participants who gave specific answers was as high as 66\% for certain questions, and the mean difference across all questions is 20\% (17\% median).
    
        \paragraph{Social Media Use}
        MTurkers were more likely to use specific social media cites as well as ``Any other social media site'' than respondents to Pew's survey. 93\% of MTurkers reported using Facebook, while only 72\% of Pew respondents did, a gap of 21\%. This gap expands to 51\%, 66\%, and 56\% respectively for Instagram, Twitter, and ``Any other social media site''.  
        
        \paragraph{Beliefs}
        MTurkers were more in favor of the right to remove personal information from public search results than Pew respondents, with MTurkers more likely 11\% to 32\% to agree about the right to remove certain types of data. \texttt{belief4}, about the right to remove ``Potentially embarrassing photos or videos'' from public search results, was the \textit{only} question across all categories for which MTurkers' answers matched Pew's representative sample ($p=0.219$), with only a 2\% difference in the rate of MTurkers' and Pew respondents answering ``Yes'' to the question.  Respondents in both Prolific samples also matched Pew respondents for \texttt{belief4}.
        
        \paragraph{Experiences}
        MTurkers were much more likely than Pew respondents to report having experienced credit/debit card fraud or account takeovers within the past 12 months. While they were somewhat similar to Pew respondents regarding the frequency with which they were asked to ``Agree to the terms and conditions of a company's privacy policy'', statistical tests find a significant difference ($p<0.001$). 
        
        \paragraph{Knowledge}
        We expand on past work by using a survey which asked knowledge questions with correct or incorrect answers, thus measuring the actual knowledge, rather than self-reported knowledge, of participants regarding several topics. MTurkers, like Prolific participants, were \textit{more confident}, in that they were much less likely to answer ``Not sure'' (5--40\% fewer ``Not sure'' answers than Pew) when asked knowledge questions. MTurkers also had a larger fraction of incorrect answers to all 8 knowledge questions (4--29\% more incorrect answers than Pew). By contrast, Prolific respondents were much more likely to produce correct answers. The distribution of MTurkers' answers (as well as Prolific respondents' answers) to all 8 knowledge questions were statistically significantly different ($p<0.001$) from Pew respondents' answer distributions for all 8 questions
        
        \paragraph{Perceptions}
        Compared to Pew respondents, MTurkers were much more comfortable with various uses of their personal data and much more confident that companies and governments would protect and not misuse personal data. Figure~\ref{fig:mturk:perceptions} shows distributions of responses to these questions by Pew and MTurk respondents, displaying a clear trend of histograms for MTurk responses being heavily weighted to the left (`Very'' or ``Somewhat'' confident/comfortable), compared to Pew's distribution. MTurkers answering all 8 Perceptions questions produced distributions of answers that were statistically distinguishable ($p<0.001$) from Pew's.
        
        

    \subsubsection{Raking}
    Our demographic raking by age, sex, education, and race failed to significantly improve the representativeness of MTurk data. Generally speaking, our raked results for MTurk have the same non-representative trends as looking at the unweighted data, including much greater social media use, greater support for the right to remove various personal information from public search results (Beliefs), higher reporting of credit/debit card fraud and account takeover (Experiences), greater confidence and less correctness about security and privacy facts (Knowledge), and greater comfort with uses of personal data data and confidence in the trustworthiness of both companies and governments in protecting their data (Perceptions). Raking does reduce the magnitude of these non-representative skews slightly (e.g., 
    
    \subsubsection{Attention Checks and CAPTCHAs Do Not Help}
    The numbers reported above represent all responses we received from MTurk while requiring participants to have previously completed at least 50 HITs with at least a 95\% accept rate. We included 
    To test the question of whether better quality data can be derived by separating high-quality, attention-paying users from bots and those not paying attention, we included two types of attention check questions to all participants, and presented half of participants with a CAPTCHA. We find that no combination of these attention checks and/or CAPTCHA requirements is sufficient to return MTurk data to a useful level of representativeness. 
    
        \paragraph{Free-Response Attention Check}
        We examined the effects of removing all respondents ($n=313/800$, 39\% of all responses) who answered our free entry question with incoherent answers or text which we found was copy-pasted from an easily accessible internet source (e.g., Wikipedia) at least 5 times across the dataset. Removing these 39\% of responses produced a dataset in which MTurkers' answers to only 2 additional questions (in addition to \texttt{belief4}) were representative of Pew's results. For all other questions, MTurkers' distribution of answers remained statistically distinct from Pew respondents pattern of answers, although on average (mean) the magnitude of misrepresentation decreased, with about 5\% less difference on average between MTurkers and Pew respondents' rates of providing each answer to each question.
        
        \paragraph{Reading Attention Check and CAPTCHAs}
        We also tested the effect of a) removing all MTurkers who failed our reading attention check question ($n=59/800$, 7\%) and b) only using data from those who were randomized to see a CAPTCHA and passed it ($n=400$). Neither of these techniques led to improved data quality, with the answers to 0 additional questions being representative when the data was quality controlled in this way. Additionally, the magnitude of difference from Pew did not change, with the mean frequency of any given answer choice across all questions remaining at about 20\%.
        
    \subsubsection{Combining Approaches}
    We also combined
    o
    
    
    
    
      Question 1 asks about frequency of being asked to agree to terms and conditions. Questions 2-4 ask about experiences with credit/debit card fraud and account takeover. Question 5 asks about familiarity with online tracking and targeting.
      
      
      . \\ VC~=~``Very Comfortable/Confident'', SC~=~``Somewhat Comfortable/Confident'', NTC~=~``Not too Comfortable/Confident'', NCAA~=~``Not Comfortable/Confident at All''
      
      
      Questions 2-5 ask about use of various social networks. Question 1 asks about choices not to use a service for privacy reasons.
     
     
     
\subsection{Even Distributions?}
Within our MTurk sample, we noticed that the distributions of answers tended to be more uniform than in Prolific. This leads us to suspect that if there is a significant number of bots on MTurk that are randomly selecting responses, we would see similar uniform distributions of answers. This also would provide an alternative explanation for the higher proportion of incorrect responses to knowledge questions on MTurk. As knowledge questions have only 1 correct answer and 1 ``Not sure'' answer but between 3-5 correct answers, it would be more likely for those who are randomly selecting answers to choose an incorrect response.

        65+: more ``Not Sure'', less social media usage, much less likely to know what private browsing is, few differences in perceptions, beliefs, similar experiences, less frequency of terms and conditions
        
        Asian: slightly more FB, Insta, much more Twitter and other social media. More familiarity with profiling/targeting, otherwise similar experiences. Mixed bag on knowledge. Generally biased toward more comfort/confidence for Perceptions. More on law enforcement data removal belief.
        
        Black: More insta, a bit more twitter. More frequent terms agreement, more experiences of fraud and account takeover. More incorrect and Not Sure in Knowledge across the board. No clear pattern in perceptions or beliefs.
        
        HS or less: Less social media usage for all apps. Less familiarity with targeting, fewer terms of service. More Not Sure, a bit more incorrect. Very similar perceptions and beliefs, somewhat higher media coverage removal.
